No Privacy Left Outside: On the (In-)Security of TEE-Shielded DNN Partition for On-Device ML

On-device ML introduces new security challenges: DNN models become white-box accessible to device users. Based on white-box information, adversaries can conduct effective model stealing (MS) and membership inference attack (MIA). Using Trusted Execution Environments (TEEs) to shield on-device DNN models aims to downgrade (easy) white-box attacks to (harder) black-box attacks. However, one major shortcoming is the sharply increased latency (up to 50X). To accelerate TEE-shield DNN computation with GPUs, researchers proposed several model partition techniques. These solutions, referred to as TEE-Shielded DNN Partition (TSDP), partition a DNN model into two parts, offloading the privacy-insensitive part to the GPU while shielding the privacy-sensitive part within the TEE. This paper benchmarks existing TSDP solutions using both MS and MIA across a variety of DNN models, datasets, and metrics. We show important findings that existing TSDP solutions are vulnerable to privacy-stealing attacks and are not as safe as commonly believed. We also unveil the inherent difficulty in deciding optimal DNN partition configurations (i.e., the highest security with minimal utility cost) for present TSDP solutions. The experiments show that such ``sweet spot'' configurations vary across datasets and models. Based on lessons harvested from the experiments, we present TEESlice, a novel TSDP method that defends against MS and MIA during DNN inference. TEESlice follows a partition-before-training strategy, which allows for accurate separation between privacy-related weights from public weights. TEESlice delivers the same security protection as shielding the entire DNN model inside TEE (the ``upper-bound'' security guarantees) with over 10X less overhead (in both experimental and real-world environments) than prior TSDP solutions and no accuracy loss.

==> tables/ennclave.tex <==

\begin{table}[]

    \caption{The accuracy of eNNclave~\cite{schlogl2020ennclave}. Averagely, the
     relative accuracy of eNNclave is only 0.66 of $M_{\rm vic}$.}
    \label{append:tbl:ennclave_accuracy}
    \begin{adjustbox}{max width=1\linewidth}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \begin{table}[]
    \begin{tabular}{@{}ccccc@{}}
    \toprule
              & CIFAR10 & CIFAR100 & STL10   & UTKFace \\ \midrule
    AlexNet   & 53.23\% & 21..44\% & 50.89\% & 58.90\% \\
    ResNet18  & 61.13\% & 42.87\%  & 62.38\% & 59.54\% \\
    ResNet34  & 61.95\% & 43.52\%  & 64.90\% & 58.86\% \\
    VGG16\_BN & 68.53\% & 44.44\%  & 75.45\% & 64.26\% \\
    VGG19\_BN & 66.47\% & 43.37\%  & 72.19\% & 64.03\% \\ \bottomrule
    \end{tabular}
    % \end{table}

\end{adjustbox}
\end{table}

==> tables/literature.tex <==

\begin{table*}[]

\caption{A summary and comparison of different model partition solutions. In each box, \cmark represents the desired attribute is satisfied and \xmark means not satisfied. \pmark means the attribute is partially satisfied and we comment the reason in the boxes.}
\label{tbl:literature}
\begin{adjustbox}{max width=1\linewidth}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \begin{table}[]
    \begin{tabular}{@{}ccccccccccc@{}}
    \toprule
    \multirow{4}{*}{Literature}                                & \multirow{4}{*}{Venue} & \multicolumn{3}{c}{Protected Attributes}                                                                                                                                                                               &  & \multicolumn{3}{c}{Defendable Attacks}                                                                                                                                                                              &  & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Benchmark \\ Category\end{tabular}}                                         \\ \cmidrule(lr){3-5} \cmidrule(lr){7-9}  
                                                               &                        & \begin{tabular}[c]{@{}c@{}}Model \\ Architecture\end{tabular} & \begin{tabular}[c]{@{}c@{}}Model \\ Weights\end{tabular}                                & \begin{tabular}[c]{@{}c@{}}Internal \\ Features\end{tabular} &  & \begin{tabular}[c]{@{}c@{}}Hardware-based\\ Stealing\end{tabular} & \begin{tabular}[c]{@{}c@{}}Gray-box \\ Retraining-based \\ Stealing\end{tabular} & \begin{tabular}[c]{@{}c@{}}Privacy \\ Inference\end{tabular} &  & \\ \midrule
    DarKnight \cite{hashemi2021darknight}     & MICRO 2021             & \xmark                                         & \xmark                                                                   & \cmark                                        &  & \xmark                                             & -                                                                                & \xmark                                        &  & -                                     \\
    Goten \cite{lucien2021goten}              & AAAI 2021              & \xmark                                         & \cmark                                                                   & \cmark                                        &  & \cmark                                             & \cmark                                                            & \cmark                                        &  & -                                     \\
    Slalom \cite{tramer2019slalom}            & ICLR 2018              & \xmark                                         & \xmark                                                                   & \cmark                                        &  & \xmark                                             & -                                                                                & \xmark                                        &  & -                                      \\
    ShadowNet \cite{sun2020shadownet}         & Arxiv 2020             & \xmark                                         & \begin{tabular}[c]{@{}c@{}}Mask \&\\ Permutation \pmark\end{tabular}     & \cmark                                        &  & \cmark                                             & \xmark                                                            & \xmark                                        &  & ShadowNet                                      \\
    Magnitude \cite{hou2021model}             & TDSC 2022              & \xmark                                         & Large-Mag. \pmark & \cmark                                        &  & \cmark                                             & \xmark                                                            & \xmark                                        &  & \begin{tabular}[c]{@{}c@{}}Shielding \\ Large-Mag. Weights\end{tabular}                                      \\
    DarkneTZ \cite{mo2020darknetz}            & MobiSys 2020           & \multicolumn{5}{c}{Last Layers \pmark}                                                                                                                                                                                                                                         & \xmark                                                            & Empirical \pmark                              &  &  \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Shielding \\ Deep Layers\end{tabular}}                                     \\
    PPFL \cite{mo2021ppfl}                    & MobiSys 2021           & \multicolumn{5}{c}{Last Layers \pmark}                                                                                                                                                                                                                                         & \xmark                                                            & Empirical \pmark                              &  &                                       \\
    Shredder \cite{mireshghallah2020shredder} & ASPLOS 2020            & \multicolumn{5}{c}{Deep Layers \pmark}                                                                                                                                                                                                                                         & \xmark                                                            & Empirical \pmark                              &  &                                       \\
    Yerbabuena \cite{gu2018yerbabuena}        & Arxiv 2018             & \multicolumn{5}{c}{Shallow Layers \pmark}                                                                                                                                                                                                                                      & \xmark                                                            & \xmark                                        &  & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Shielding \\ Shallow Layers\end{tabular}}                                       \\
    Serdab \cite{elgamal2020serdab}           & CCGRID 2020                                                & \multicolumn{5}{c}{Shallow Layers \pmark}                                                                                                                                                                                                                                         & \xmark                                                & \xmark           &  &  \\
    Origami \cite{narra2019origami}           & Arxiv 2019             & \multicolumn{5}{c}{Shallow Layers \pmark}                                                                                                                                                                                                                                      & \xmark                                                            & \cmark                                        &  &                                       \\
    AegisDNN \cite{xiang2021aegisdnn}         & RTSS 2021              & \multicolumn{5}{c}{Partial Layers \pmark}                                                                                                                                                                                                                                      & \xmark                                                            & \xmark                                        &  &  SOTER                                     \\
    SOTER \cite{shen2022soter}                & \footnotesize{USENIX ATC 2022} & \multicolumn{5}{c}{Partial Layers \& Weight Morph \pmark}                                                                                                                                                                                                                         & \xmark                                                & \xmark           &  &  \\
    GINN \cite{asvadishirehjini2022ginn}      & \footnotesize{CODASPY 2022}           & \xmark                                         & \xmark                                                                   & \xmark                                        &  & \xmark                                             & -                                                                                & \xmark                                        &  & -                                      \\
    eNNclave \cite{schlogl2020ennclave}       & AISec 2020                                                 & \xmark                                         & \cmark                                                                      & \cmark                                        &  & \cmark                                             & \cmark                                                & \cmark           &  & - \\
    Ours                                                       & -                      & \cmark                                         & \cmark                                                                   & \cmark                                        &  & \cmark                                             & \cmark                                                            & \cmark                                        &  & -                                      \\ \bottomrule
    \end{tabular}
    % \end{table}
\end{adjustbox}
\end{table*}

==> tables/literature_with_assumption.tex <==

\begin{table*}[]

\caption{A summary and comparison of different model partition solutions. In each box, \cmark represents the desired attribute is satisfied and \xmark means not satisfied. \pmark means the attribute is partially satisfied and we comment the reason in the boxes.}
\label{tbl:literature}
\begin{adjustbox}{max width=1\linewidth}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \begin{table}[]
    \begin{tabular}{@{}ccccccccccccc@{}}
    \toprule
    \multirow{4}{*}{Literature}                                & \multirow{4}{*}{Venue} & \multicolumn{3}{c}{Protected Attributes}                                                                                                                                                                               &  & \multicolumn{3}{c}{Defendable Attacks}                                                                                                                                                                              &  & Defender Assumption & & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Benchmark \\ Category\end{tabular}}                                         \\ \cmidrule(lr){3-5} \cmidrule(lr){7-9} \cmidrule(lr){11-11} 
                                                               &                        & \begin{tabular}[c]{@{}c@{}}Model \\ Architecture\end{tabular} & \begin{tabular}[c]{@{}c@{}}Model \\ Weights\end{tabular}                                & \begin{tabular}[c]{@{}c@{}}Internal \\ Features\end{tabular} &  & \begin{tabular}[c]{@{}c@{}}Hardware-based\\ Stealing\end{tabular} & \begin{tabular}[c]{@{}c@{}}Gray-box \\ Retraining-based \\ Stealing\end{tabular} & \begin{tabular}[c]{@{}c@{}}Privacy \\ Inference\end{tabular} &  & \begin{tabular}[c]{@{}c@{}}One \\ Trusty Party\end{tabular} & & \\ \midrule
    DarKnight \cite{hashemi2021darknight}     & MICRO 2021             & \xmark                                         & \xmark                                                                   & \cmark                                        &  & \xmark                                             & -                                                                                & \xmark                                        &  & \xmark &  & -                                     \\
    Goten \cite{lucien2021goten}              & AAAI 2021              & \xmark                                         & \cmark                                                                   & \cmark                                        &  & \cmark                                             & \cmark                                                            & \cmark                                        &  & \xmark &  & -                                     \\
    Slalom \cite{tramer2019slalom}            & ICLR 2018              & \xmark                                         & \xmark                                                                   & \cmark                                        &  & \xmark                                             & -                                                                                & \xmark                                        &  & \cmark &  & -                                      \\
    ShadowNet \cite{sun2020shadownet}         & Arxiv 2020             & \xmark                                         & \begin{tabular}[c]{@{}c@{}}Mask \&\\ Permutation \pmark\end{tabular}     & \cmark                                        &  & \cmark                                             & \xmark                                                            & \xmark                                        &  & \cmark &  & ShadowNet                                      \\
    Magnitude \cite{hou2021model}             & TDSC 2022              & \xmark                                         & Large-Mag. \pmark & \cmark                                        &  & \cmark                                             & \xmark                                                            & \xmark                                        &  & \cmark &  & \begin{tabular}[c]{@{}c@{}}Shielding \\ Large-Mag. Weights\end{tabular}                                      \\
    DarkneTZ \cite{mo2020darknetz}            & MobiSys 2020           & \multicolumn{5}{c}{Last Layers \pmark}                                                                                                                                                                                                                                         & \xmark                                                            & Empirical \pmark                              &  & \cmark &  &  \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Shielding \\ Deep Layers\end{tabular}}                                     \\
    PPFL \cite{mo2021ppfl}                    & MobiSys 2021           & \multicolumn{5}{c}{Last Layers \pmark}                                                                                                                                                                                                                                         & \xmark                                                            & Empirical \pmark                              &  & \cmark &  &                                       \\
    Shredder \cite{mireshghallah2020shredder} & ASPLOS 2020            & \multicolumn{5}{c}{Deep Layers \pmark}                                                                                                                                                                                                                                         & \xmark                                                            & Empirical \pmark                              &  & \cmark &  &                                       \\
    Yerbabuena \cite{gu2018yerbabuena}        & Arxiv 2018             & \multicolumn{5}{c}{Shallow Layers \pmark}                                                                                                                                                                                                                                      & \xmark                                                            & \xmark                                        &  & \cmark &  & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Shielding \\ Shallow Layers\end{tabular}}                                       \\
    Serdab \cite{elgamal2020serdab}           & CCGRID 2020                                                & \multicolumn{5}{c}{Shallow Layers \pmark}                                                                                                                                                                                                                                         & \xmark                                                & \xmark           &  & \cmark &  &  \\
    Origami \cite{narra2019origami}           & Arxiv 2019             & \multicolumn{5}{c}{Shallow Layers \pmark}                                                                                                                                                                                                                                      & \xmark                                                            & \cmark                                        &  & \cmark &  &                                       \\
    AegisDNN \cite{xiang2021aegisdnn}         & RTSS 2021              & \multicolumn{5}{c}{Partial Layers \pmark}                                                                                                                                                                                                                                      & \xmark                                                            & \xmark                                        &  & \cmark &  &  SOTER                                     \\
    SOTER \cite{shen2022soter}                & \footnotesize{USENIX ATC 2022} & \multicolumn{5}{c}{Partial Layers \& Weight Morph \pmark}                                                                                                                                                                                                                         & \xmark                                                & \xmark           &  & \cmark &  &  \\
    GINN \cite{asvadishirehjini2022ginn}      & \footnotesize{CODASPY 2022}           & \xmark                                         & \xmark                                                                   & \xmark                                        &  & \xmark                                             & -                                                                                & \xmark                                        &  & \cmark &  & -                                      \\
    eNNclave \cite{schlogl2020ennclave}       & AISec 2020                                                 & \xmark                                         & \cmark                                                                      & \cmark                                        &  & \cmark                                             & \cmark                                                & \cmark           &  & \cmark &  & - \\
    Ours                                                       & -                      & \cmark                                         & \cmark                                                                   & \cmark                                        &  & \cmark                                             & \cmark                                                            & \cmark                                        &  & \cmark &  & -                                      \\ \bottomrule
    \end{tabular}
    % \end{table}
\end{adjustbox}
\end{table*}

==> tex/append_sec/ennclave.tex <==
\section{Accuracy of eNNclave}
\label{append:sec:ennclave}

To quantitatively understand the accuracy loss of
eNNclave~\cite{schlogl2020ennclave}, we implement their framework in all the
settings of our benchmark. We use the recommended configuration of the original
paper, \ie, putting $M_{\rm vic}$'s last layer into TEE while replacing the
GPU-offloaded shallow layers with a public backbone. The accuracy is summarized
in \T~\ref{append:tbl:ennclave_accuracy}. It can be observed that the accuracy
is much lower than $M_{\rm vic}$ and \sys of \T~\ref{tbl:nettailor_accuracy}.
The average relative ratio of eNNclave compared to the accuracy of $M_{\rm vic}$ is only 0.66.

\input{tables/ennclave.tex}


==> tex/append_sec/other_metrics_two_figs.tex <==

\section{Results on Other Metrics}
\label{append:sec:other_metrics_two_figs}

As noted in our main paper, when assessing the security of existing \tsdp\
solutions, we consider seven metrics. This Appendix section will
re-visit the employed $Security$ metrics and then display the results of
the other $Security$ metrics. 

In \F~\ref{fig:acc_flops_append_one_fig}, we display the accuracy, fidelity, and
ASR for all the models and datasets. In \F~\ref{fig:mia_flops_append_one_fig},
we displayed the confidence-based attack accuracy, gradient-based attack
accuracy, generalization gap, and confidence gap. 

\begin{figure*}[!ht]
\centering
\includegraphics[width=\linewidth]{figs/acc_flops_standard_five_models_one_fig.pdf}
\caption{Model stealing results in terms of accuracy, fidelity, and ASR.}
\label{fig:acc_flops_append_one_fig}
\end{figure*} 

\begin{figure*}[!ht]
\centering
\includegraphics[width=\linewidth]{figs/mia_flops_standard_five_models_one_fig.pdf}
\caption{Membership inference results of generalization gap, confidence gap, confidence-based membership inference attack accuracy, and gradient-based membership inference attack accuracy.}
\label{fig:mia_flops_append_one_fig}
\end{figure*} 


The results are consistent with the results in
the main paper. The tendencies of curves are generally consistent with the
conclusions in the main paper. 



==> tex/append_sec/visualization.tex <==
\section{Analysis of Slices}
\label{sec:append:visualization}


\begin{figure}[!t]
    \centering
    \includegraphics[width=0.8\linewidth]{ppt/visualization.pdf}
    \vspace{-6pt}
    \caption{The visualization of three hybrid models.}
    \label{fig:nettailor_vis}
    \vspace{-10pt}

    \end{figure} 

\parh{Visualization.}~In \F~\ref{fig:nettailor_vis}, we plot three hybrid models
to provide an intuitive understanding of the extracted slices. As illustrated,
most slices skip one block of the ResNet model. It means the slices work like a
residual function of the blocks~\cite{he2016deep}. The hybrid model of VGG16\_BN
has more slices than the ResNet models. This is because the VGG model (the
victim model) is less similar to ResNet18 (the backbone) than any other ResNet
model. Although the number of slices is comparable to or even larger than the
number of blocks in the figure, the total computation cost (FLOPs) of slices is
much smaller than that of the backbone. It is because each slice is designed to
be lightweight (about 18$\times$ smaller than the layer) and performs only a
small amount of computation.

\parh{Slice Allocation.}~\F~\ref{fig:nettailor_vis} illustrates that the slices
created by \tool\ locate across the entire backbone, from shallow to deep
layers. Accordingly, the weights of all the backbone layers need to be adjusted.
This observation explains the relatively low accuracy of
eNNclave~\cite{schlogl2020ennclave}, given that it only changes the deep layers
and uses the public backbone's shallow layers directly. 


==> tex/literature.tex <==
\subsection{Literature Review}



\subsection{Limitation}
\label{sec:literature:limitation}

After conceptually reviewing the characteristics of prior works, we found that there are ten solutions that can protect model functionalities under our threat model. The other five works in Table~\ref{tbl:literature} can not be applied to our scenario because some do not protect model weights (DarKnight~\cite{hashemi2021darknight}, Slalom~\cite{tramer2019slalom}, and GINN~\cite{asvadishirehjini2022ginn}), some have stronger defender assumption (Goten~\cite{lucien2021goten}), and some significantly sacrifice DNN accuracy (eNNclave~\cite{schlogl2020ennclave}). We divide the ten available solutions into five categories:
\begin{itemize}
    \item Shielding Deep Layers: DarkneTZ~\cite{mo2020darknetz}, PPFL~\cite{mo2021ppfl}, and Shredder~\cite{mireshghallah2020shredder}. 
    \item Shielding Shallow Layers: Yerbabuena~\cite{gu2018yerbabuena}, Origami~\cite{narra2019origami}, and Serdab~\cite{elgamal2020serdab}.
    \item Shielding Large-Magnitude Weights: \cite{hou2021model}.
    \item Shielding Intermediate Layers: AegisDNN~\cite{xiang2021aegisdnn} and SOTER~\cite{shen2022soter}. 
    \item Shielding Non-Linear Layers: ShadowNet~\cite{sun2020shadownet}.
\end{itemize}
For these approaches, we found that there are several challenges to understanding their security guarantee and comparing different solutions.

\textbf{Different Experimental Settings.}
The experimental settings in different works are different. For example, DarkneTZ~\cite{mo2020darknetz} and ShadowNet~\cite{sun2020shadownet} use completely different models in the experiments. Even for the models from the same family, the implementations may be different. Both DarkneTZ~\cite{mo2020darknetz} and PPFL~\cite{mo2021ppfl} evaluate VGG models, but the specific architectures are different.

\textbf{Different Evaluated Attacks.}
The evaluated attacks of different work are different. Prior work either reported the defense result against stealing attacks or privacy inference attacks. \textbf{No} paper shows the defense against two attacks at the same time. DarkneTZ~\cite{mo2020darknetz} and PPFL~\cite{mo2021ppfl} only report the empirical evaluation on privacy protection. \cite{hou2021model} and ShadowNet~\cite{sun2020shadownet} report the result against stealing attacks. It is difficult to understand the defense effectiveness across different attacks.

\textbf{Manual Configuration.}
The defender needs to manually configure the partition strategy for different models and tasks. For example, Shredder~\cite{mireshghallah2020shredder} and Yerbabuena~\cite{gu2018yerbabuena} give different optimal model partition settings for different models. It is difficult to apply such configurations to new models and datasets.

\textbf{No Theoretical Guarantee.}
Several protection schemes are built on empirical observation and set empirical thresholds. It remains doubtful how much security can such schemes provide. For example, DarkneTZ~\cite{mo2020darknetz} and PPFL~\cite{mo2021ppfl} claim that putting the last layer inside TEE is enough. \cite{hou2021model} observed that protecting the largest-magnitude 1\% weights can defend against model stealing attacks.

